Moderating New Waves of Online Hate with Chain-of-Thought Reasoning in Large Language Models

Online hate is an escalating problem that negatively impacts the lives of Internet users, and is also subject to rapid changes due to evolving events, resulting in new waves of online hate that pose a critical threat. Detecting and mitigating these new waves present two key challenges: it demands reasoning-based complex decision-making to determine the presence of hateful content, and the limited availability of training samples hinders updating the detection model. To address this critical issue, we present a novel framework called HATEGUARD for effectively moderating new waves of online hate. HATEGUARD employs a reasoning-based approach that leverages the recently introduced chain-of-thought (CoT) prompting technique, harnessing the capabilities of large language models (LLMs). HATEGUARD further achieves prompt-based zero-shot detection by automatically generating and updating detection prompts with new derogatory terms and targets in new wave samples to effectively address new waves of online hate. To demonstrate the effectiveness of our approach, we compile a new dataset consisting of tweets related to three recently witnessed new waves: the 2022 Russian invasion of Ukraine, the 2021 insurrection of the US Capitol, and the COVID-19 pandemic. Our studies reveal crucial longitudinal patterns in these new waves concerning the evolution of events and the pressing need for techniques to rapidly update existing moderation tools to counteract them. Comparative evaluations against state-of-the-art tools illustrate the superiority of our framework, showcasing a substantial 22.22% to 83.33% improvement in detecting the three new waves of online hate. Our work highlights the severe threat posed by the emergence of new waves of online hate and represents a paradigm shift in addressing this threat practically.

==> backup.tex <==
%------------------------------------------------------------------------
\begin{table*}[t!]
\begin{tabular}{c|c|cc|cc|cc|cc}
\specialrule{1pt}{0pt}{-1pt}
\multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Q1 (Jan2020 - Mar2020)}}                                                                                        & \multicolumn{2}{c|}{\textbf{Q2 (Apr2020 - Jun2020)}}                                                                                        & \multicolumn{2}{c|}{\textbf{Q3 (Jul2020 - Sep2020)}}                                                                                        & \multicolumn{2}{c}{\textbf{Q4 (Oct2020 - Dec2020)}}                                                                                        \\ \cline{3-10} 
                                   &                                  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Before\\ deploying\end{tabular}} & \begin{tabular}[c]{@{}c@{}}After\\ deploying\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Before\\ deploying\end{tabular}} & \begin{tabular}[c]{@{}c@{}}After\\ deploying\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Before\\ deploying\end{tabular}} & \begin{tabular}[c]{@{}c@{}}After\\ deploying\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Before\\ deploying\end{tabular}} & \begin{tabular}[c]{@{}c@{}}After\\ deploying\end{tabular} \\ \hline
\multirow{4}{*}{Asian}             & \ProjectName{}                              & \multicolumn{1}{c|}{\multirow{4}{*}{52}}                                        & 15                                                        & \multicolumn{1}{c|}{\multirow{4}{*}{122}}                                       & 23                                                        & \multicolumn{1}{c|}{\multirow{4}{*}{244}}                                       & 65                                                        & \multicolumn{1}{c|}{\multirow{4}{*}{181}}                                       & 46                                                        \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} 
                                   & Transformer (Bert)               & \multicolumn{1}{c|}{}                                                           & 37                                                        & \multicolumn{1}{c|}{}                                                           & 71                                                        & \multicolumn{1}{c|}{}                                                           & 132                                                       & \multicolumn{1}{c|}{}                                                           & 100                                                       \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} 
                                   & FSL                              & \multicolumn{1}{c|}{}                                                           & 26                                                        & \multicolumn{1}{c|}{}                                                           & 33                                                        & \multicolumn{1}{c|}{}                                                           & 104                                                       & \multicolumn{1}{c|}{}                                                           & 74                                                        \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} 
                                   & Meta-FSL                         & \multicolumn{1}{c|}{}                                                           & 20                                                        & \multicolumn{1}{c|}{}                                                           & 79                                                        & \multicolumn{1}{c|}{}                                                           & 105                                                       & \multicolumn{1}{c|}{}                                                           & 79                                                        \\ \hline
\multirow{4}{*}{Mask}              & \ProjectName{}                                & \multicolumn{1}{c|}{\multirow{4}{*}{10}}                                        & 0                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{37}}                                        & 3                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{42}}                                        & 5                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{177}}                                       & 14                                                        \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} 
                                   & Transformer (Bert)               & \multicolumn{1}{c|}{}                                                           & 3                                                         & \multicolumn{1}{c|}{}                                                           & 17                                                        & \multicolumn{1}{c|}{}                                                           & 22                                                        & \multicolumn{1}{c|}{}                                                           & 55                                                        \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} 
                                   & FSL                              & \multicolumn{1}{c|}{}                                                           & 2                                                         & \multicolumn{1}{c|}{}                                                           & 17                                                        & \multicolumn{1}{c|}{}                                                           & 17                                                        & \multicolumn{1}{c|}{}                                                           & 46                                                        \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} 
                                   & Meta-FSL                         & \multicolumn{1}{c|}{}                                                           & 7                                                         & \multicolumn{1}{c|}{}                                                           & 22                                                        & \multicolumn{1}{c|}{}                                                           & 29                                                        & \multicolumn{1}{c|}{}                                                           & 73                                                        \\ \hline
\multirow{4}{*}{Vaccine}           & \ProjectName{}                                & \multicolumn{1}{c|}{\multirow{4}{*}{10}}                                        & 2                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{46}}                                        & 3                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{52}}                                        & 4                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{87}}                                        & 9                                                         \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} 
                                   & Transformer (Bert)               & \multicolumn{1}{c|}{}                                                           & 6                                                         & \multicolumn{1}{c|}{}                                                           & 11                                                        & \multicolumn{1}{c|}{}                                                           & 19                                                        & \multicolumn{1}{c|}{}                                                           & 30                                                        \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} 
                                   & FSL                              & \multicolumn{1}{c|}{}                                                           & 3                                                         & \multicolumn{1}{c|}{}                                                           & 12                                                        & \multicolumn{1}{c|}{}                                                           & 14                                                        & \multicolumn{1}{c|}{}                                                           & 21                                                        \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} 
                                   & Meta-FSL                         & \multicolumn{1}{c|}{}                                                           & 6                                                         & \multicolumn{1}{c|}{}                                                           & 35                                                        & \multicolumn{1}{c|}{}                                                           & 24                                                        & \multicolumn{1}{c|}{}                                                           & 38                                                        \\ \hline
\multirow{4}{*}{Boomer}            & \ProjectName{}                              & \multicolumn{1}{c|}{\multirow{4}{*}{0}}                                         & -                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{0}}                                         & -                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{13}}                                        & 6                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{132}}                                       & 46                                                        \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} 
                                   & Transformer (Bert)               & \multicolumn{1}{c|}{}                                                           & -                                                         & \multicolumn{1}{c|}{}                                                           & -                                                         & \multicolumn{1}{c|}{}                                                           & 12                                                        & \multicolumn{1}{c|}{}                                                           & 92                                                        \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} 
                                   & FSL                              & \multicolumn{1}{c|}{}                                                           & -                                                         & \multicolumn{1}{c|}{}                                                           & -                                                         & \multicolumn{1}{c|}{}                                                           & 5                                                         & \multicolumn{1}{c|}{}                                                           & 69                                                        \\ \cline{2-2} \cline{4-4} \cline{6-6} \cline{8-8} \cline{10-10} 
                                   & Meta-FSL                         & \multicolumn{1}{c|}{}                                                           & -                                                         & \multicolumn{1}{c|}{}                                                           & -                                                         & \multicolumn{1}{c|}{}                                                           & 6                                                         & \multicolumn{1}{c|}{}                                                           & 73                                                        \\ 
\specialrule{1pt}{0pt}{-1pt}
\end{tabular}
\vspace{1mm}
\caption{Violation checking through different methods.}
\label{tab:violations}
\end{table*}

%------------------------------------------------------------------------
\begin{table}[ht]
\centering
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\specialrule{1.6pt}{0pt}{-1pt}
\textbf{Category}        & \textbf{Method} & \textbf{\begin{tabular}[c]{@{}c@{}}Q1 (Jan2020\\ - Mar2020)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Q2 (Apr2020\\ - Jun2020)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Q3 (Jul2020\\ - Sep2020)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Q4 (Oct2020\\ - Dec2020)\end{tabular}} \\ \hline
\multirow{3}{*}{Asian}   & FSL             & 0.66                                                                      & 0.84                                                                      & 0.71                                                                      & 0.74                                                                      \\ \cline{2-6} 
                         & Meta-FSL        & 0.74                                                                      & 0.74                                                                      & 0.71                                                                      & 0.71                                                                      \\ \cline{2-6} 
                         & Our             & \textbf{0.84}                                                             & \textbf{0.88}                                                             & \textbf{0.81}                                                             & \textbf{0.83}                                                             \\ \hline
\multirow{3}{*}{Mask}    & FSL             & \textbf{0.89}                                                             & 0.49                                                                      & 0.6                                                                       & 0.72                                                                      \\ \cline{2-6} 
                         & Meta-FSL        & 0.43                                                                      & 0.46                                                                      & 0.41                                                                      & 0.68                                                                      \\ \cline{2-6} 
                         & Our             & 0.8                                                                       & \textbf{0.65}                                                             & \textbf{0.77}                                                             & \textbf{0.75}                                                             \\ \hline
\multirow{3}{*}{Vaccine} & FSL             & 0.56                                                                      & 0.37                                                                      & \textbf{0.7}                                                              & \textbf{0.73}                                                             \\ \cline{2-6} 
                         & Meta-FSL        & 0.5                                                                       & 0.58                                                                      & 0.63                                                                      & 0.68                                                                      \\ \cline{2-6} 
                         & Our             & \textbf{0.65}                                                             & \textbf{0.65}                                                             & 0.64                                                                      & 0.71                                                                      \\ \hline
\multirow{3}{*}{Boomer}  & FSL             & -                                                                         & -                                                                         & \textbf{0.76}                                                             & 0.61                                                                      \\ \cline{2-6} 
                         & Meta-FSL        & -                                                                         & -                                                                         & 0.47                                                                      & 0.51                                                                      \\ \cline{2-6} 
                         & Our             & -                                                                         & -                                                                         & 0.73                                                                      & \textbf{0.74 }                                                                     \\ \hline
\specialrule{1pt}{0pt}{-1pt}
\end{tabular}%
}
\vspace{1mm}
\caption{F1-score through different entailment strategies.}
\label{tab:entailments}
\end{table}

%------------------------------------------------------------------------
\begin{table}[ht]
\centering
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\specialrule{1.6pt}{0pt}{-1pt}
\textbf{Category}        & \textbf{Method} & \textbf{\begin{tabular}[c]{@{}c@{}}Q1 (Jan2020\\ - Mar2020)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Q2 (Apr2020\\ - Jun2020)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Q3 (Jul2020\\ - Sep2020)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Q4 (Oct2020\\ - Dec2020)\end{tabular}} \\ \hline
\multirow{3}{*}{Asian}   & FSL             & 0.66                                                                      & 0.84                                                                      & 0.71                                                                      & 0.74                                                                      \\ \cline{2-6} 
                         & Meta-FSL        & 0.74                                                                      & 0.74                                                                      & 0.71                                                                      & 0.71                                                                      \\ \cline{2-6} 
                         & Our             & \textbf{0.84}                                                             & \textbf{0.88}                                                             & \textbf{0.81}                                                             & \textbf{0.83}                                                             \\ \hline
\multirow{3}{*}{Mask}    & FSL             & \textbf{0.89}                                                             & 0.49                                                                      & 0.6                                                                       & 0.72                                                                      \\ \cline{2-6} 
                         & Meta-FSL        & 0.43                                                                      & 0.46                                                                      & 0.41                                                                      & 0.68                                                                      \\ \cline{2-6} 
                         & Our             & 0.8                                                                       & \textbf{0.65}                                                             & \textbf{0.77}                                                             & \textbf{0.75}                                                             \\ \hline
\multirow{3}{*}{Vaccine} & FSL             & 0.56                                                                      & 0.37                                                                      & \textbf{0.7}                                                              & \textbf{0.73}                                                             \\ \cline{2-6} 
                         & Meta-FSL        & 0.5                                                                       & 0.58                                                                      & 0.63                                                                      & 0.68                                                                      \\ \cline{2-6} 
                         & Our             & \textbf{0.65}                                                             & \textbf{0.65}                                                             & 0.64                                                                      & 0.71                                                                      \\ \hline
\multirow{3}{*}{Boomer}  & FSL             & -                                                                         & -                                                                         & \textbf{0.76}                                                             & 0.61                                                                      \\ \cline{2-6} 
                         & Meta-FSL        & -                                                                         & -                                                                         & 0.47                                                                      & 0.51                                                                      \\ \cline{2-6} 
                         & Our             & -                                                                         & -                                                                         & 0.73                                                                      & \textbf{0.74 }                                                                     \\ \hline
\specialrule{1pt}{0pt}{-1pt}
\end{tabular}%
}
\vspace{1mm}
\caption{F1-score through different entailment strategies.}
\label{tab:entailments}
\end{table}

%------------------------------------------------------------------------
\begin{table}[ht]
\centering
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c}
\specialrule{1pt}{0pt}{-1pt}
\textbf{Category}            & \textbf{Data Size}   & \textbf{Method} & \textbf{Violations} & \textbf{F1-Score} \\ \hline
\multirow{2}{*}{Asian}       & \multirow{2}{*}{200} & MMBT            & 125                 & 0.28              \\ \cline{3-5} 
                             &                      & Our             & \textbf{57}         & \textbf{0.65}     \\ \hline
\multirow{2}{*}{Ageisom}     & \multirow{2}{*}{200} & MMBT            & 161                 & 0.18              \\ \cline{3-5} 
                             &                      & Our             & \textbf{42}         & \textbf{0.67}     \\ \hline
\multirow{2}{*}{Vaccine}     & \multirow{2}{*}{98}  & MMBT            & 67                  & 0.3               \\ \cline{3-5} 
                             &                      & Our             & \textbf{21}         & \textbf{0.54}     \\ \hline
\multirow{2}{*}{Immigration} & \multirow{2}{*}{54}  & MMBT            & 41                  & 0.19              \\ \cline{3-5} 
                             &                      & Our             & \textbf{22}         & \textbf{0.62}     \\ \hline
\multirow{2}{*}{Election}    & \multirow{2}{*}{200} & MMBT            & 92                  & 0.36              \\ \cline{3-5} 
                             &                      & Our             & \textbf{35}         & \textbf{0.64}     \\ 
\specialrule{1pt}{0pt}{-1pt}
\end{tabular}%
}
\vspace{1mm}
\caption{Evaluation for Hateful Memes}
\label{tab:memes}
\end{table}

==> baseline_table.tex <==
% This table compare the baseline with \ProjectNameTable{} framework
%\vspace{-4mm}
% \begin{table*}[t]
% \centering
% \resizebox{0.94\textwidth}{!}{%
% % \setlength\tabcolsep{0.1ex}
% \begin{tabular}{cccccccccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Q1 (Jan-Mar)}} & \multicolumn{3}{c}{\textbf{Q2 (Apr-Jun)}} & \multicolumn{3}{c}{\textbf{Q3 (Jul-Sep)}} & \multicolumn{3}{c}{\textbf{Q4 (Oct-Dec)}} \\
% \cmidrule(r){3-5} \cmidrule(r){6-8} \cmidrule(r){9-11} \cmidrule(r){12-14}                                                                                  &                                  & \textbf{\begin{tabular}[c]{@{}c@{}}\# of\\ Hateful\\ Sample\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Viola-\\ tion\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Improv-\\ ement\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# of\\ Hateful\\ Sample\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Viola-\\ tion\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Improv-\\ ement\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# of\\ Hateful\\ Sample\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Viola-\\ tion\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Improv-\\ ement\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# of\\ Hateful\\ Sample\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Viola-\\ tion\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Improv-\\ ement\end{tabular}} \\
% \midrule                                                                                 
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Ageism\\ (2020)\end{tabular}}         & \ProjectNameTable{}                              & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}293/\\ 2,195\end{tabular}}     & \textbf{58} & -  
% & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}228/\\ 1,120\end{tabular}}     & \textbf{41} & - & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}232/\\ 981\end{tabular}}       & \textbf{47} & - & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}316/\\ 856\end{tabular}}       & \textbf{66} & - \\
%  & BERT-base & & 177 & 67.2\% & & 93 &    55.9\% & & 108 & 56.5\% & & 91 & 27.5\% \\
%  & Tweet-NLP & & 196 & 70.4\% & & 114 & 64\% & & 120 & 60.8\% & & 102 & 35.3\% 
%  \\
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Asian\\ (2020)\end{tabular}}          & \ProjectNameTable{}                              & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}427/\\ 1,035\end{tabular}}     & \textbf{76} &            -                                                      & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}683/\\ 1,760\end{tabular}}     & \textbf{115}                                                   &                    -                                              & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}744/\\ 1,678\end{tabular}}     & \textbf{144} &                            -                                      & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}578/\\ 1,163\end{tabular}}     & \textbf{109} &               -
% \\
%  & BERT-base & & 168 & 54.8\% & & 261 & 55.9\% & & 231 & 37.7\% & & 162 & 32.7\%
%  \\
%  & Tweet-NLP & & 170 & 55.3\% & & 230 & 50\% & & 272 & 47.1\% & & 181 & 39.8\%
%  \\
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Mask\\ (2020)\end{tabular}}           & \ProjectNameTable{}                              & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}18/\\ 149\end{tabular}}        & \textbf{2}                                                     &                                  -                                & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}109/\\ 841\end{tabular}}       & \textbf{17}                                                    &                                                  -                & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}383/\\ 2,784\end{tabular}}     & \textbf{34}                                                    &         -                                                         & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}342/\\ 1,679\end{tabular}}     & \textbf{26}                                                    &      -
% \\
% & BERT-base & & 7 & 71.4\% & & 54 & 68.5\% & & 202 & 83.2\% & & 112 & 76.8\%
% \\
% & Tweet-NLP & & 10 & 80\% & & 61 & 72.1\% & & 205 & 83.4\% & & 107 & 75.7\%
% \\
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Vaccine\\ (2020)\end{tabular}}        & \ProjectNameTable{} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}119/\\ 817\end{tabular}}       & \textbf{11} & - & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}160/\\ 1,118\end{tabular}}     & \textbf{12} & - & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}176/\\ 1,056\end{tabular}}     & \textbf{19} & - & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}361/\\ 2,391\end{tabular}}     & \textbf{38} & -
% \\
%  & BERT-base & & 56 & 80.4\% & & 79 & 84.8\% & & 78 & 75.6\% & & 141 & 73\% \\
%  & Tweet-NLP & & 72 & 84.7\% & & 71 & 83.1\% & & 85 & 77.6\% & & 137 & 72.3\% \\
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}US Capitol\\ (2021)\end{tabular}}     & \ProjectNameTable{}                              & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}767/\\ 2,519\end{tabular}}     & \textbf{129} & - & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}201/\\ 624\end{tabular}}       & \textbf36 & - & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}320/\\ 904\end{tabular}} & \textbf{52} & - & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}265/\\ 817\end{tabular}}       & \textbf{39} & -
% \\
%  & BERT-base & & 370 & 65.1\% & & 93 & 61.3\% & & 121 & 57\% & & 115 & 66.1\% 
%  \\
%  & Tweet-NLP & & 446 & 71.1\% & & 83 & 56.6\% & & 177 & 70.6\% & & 134 & 71.5\% 
%  \\
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Russia-Ukraine\\ (2022)\end{tabular}} & \ProjectNameTable{}                              & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}349/\\ 1,828\end{tabular}}     & \textbf{94}                                                    &                              -                                    & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}311/\\ 1,383\end{tabular}}     & \textbf{78}                                                    &      -                                                            & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}432/\\ 1,313\end{tabular}}     & \textbf{89} &                                      -                            & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}127/\\ 450\end{tabular}}       & \textbf{30}                                                    &      -                                                           \\
%  & BERT-base & & 194 & 51.5\% & & 150 & 48\% & & 163 & 45.4\% & & 52 & 42.3\% 
%  \\
%  & Tweet-NLP & & 223 & 57.8\% & & 159 & 50.9\% & & 250 & 64.4\% & & 63 & 52.4\% 
%  \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Violation checking against the benchmarks. }
% \vspace{-5mm}
% \label{tab:violations_compare_baseline}
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\resizebox{1\textwidth}{!}{%
% % \setlength\tabcolsep{0.7ex}
% \begin{tabular}{cccccccccccccccccc}
% \toprule
% \multirow{3}{*}{\textbf{Wave Type}}                                                           & \multirow{3}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Quarter 1 (Jan-Mar)}}                                                                    & \multicolumn{4}{c}{\textbf{Quarter 2 (Apr-Jun)}}                                                                       & \multicolumn{4}{c}{\textbf{Quarter 3 (Jul-Sep})}                                                                    & \multicolumn{4}{c}{\textbf{Quarter 4 (Oct-Dec)}}                                                                       \\
% \cmidrule(r){3-6} \cmidrule(r){7-10} \cmidrule(r){11-14} \cmidrule(r){15-18}     
%                                                                                     &                         & \textbf{\begin{tabular}[c]{@{}c@{}}\# of\\ Tweets\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Acc-\\ uracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Prec-\\ ision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rec-\\ all\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# of\\ Tweets\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Acc-\\ uracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Prec-\\ ision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rec-\\ all\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# of\\ Tweets\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Acc-\\ uracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Prec-\\ ision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rec-\\ all\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# of\\ Tweets\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Acc-\\ uracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Prec-\\ ision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rec-\\ all\end{tabular}} \\
% \midrule
% \multicolumn{18}{c}{\textbf{- Overall Results -}}\\
% \midrule
% \multirow{3}{*}{
% \begin{tabular}[c]{@{}c@{}}Total\\ (2020-2022)\end{tabular}
% } 
% & \ProjectNameTable{} & \multirow{3}{*}{928} & \textbf{0.99} & \textbf{0.96}    & \textbf{1} & 
% \multirow{3}{*}{893} & \textbf{0.98} & \textbf{0.96} & \textbf{0.99}    
% & \multirow{3}{*}{1148} & \textbf{0.99} & \textbf{0.97} & \textbf{1} & 
% \multirow{3}{*}{1031} & \textbf{0.99}    & \textbf{0.98}    & \textbf{0.99}    \\
% & BERT-base & & 0.74 & 0.81& 0.34& & 0.82& 0.76& 0.71& &0.84 & 0.82& 0.79& & 0.83& 0.86&0.8 \\
% & Tweet-NLP & &0.7 &0.73 &0.23 & & 0.83&0.79 &0.77 & &0.84 & 0.83& 0.8& &0.83 &0.84 &0.8 \\
% \midrule
% \multicolumn{18}{c}{\textbf{- Category-wise Results -}}\\
% \midrule
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Ageism\\ (2020)\end{tabular}}            & \ProjectNameTable{}                       & \multirow{3}{*}{186}                                   & \textbf{0.99} & \textbf{0.97} & \textbf{1} & \multirow{3}{*}{117}                                   & \textbf{1}    & \textbf{1}    & \textbf{1}    & \multirow{3}{*}{114}                                   & \textbf{1}    & \textbf{1}    & \textbf{1} & \multirow{3}{*}{161}                                   & \textbf{1}    & \textbf{1}    & \textbf{1}    \\
%                                                                                     & BERT-base               &                                                        & 0.82          & 0.6           & 0.44       &                                                        & 0.8           & 0.68          & 0.53          &                                                        & 0.79          & 0.68          & 0.6        &                                                        & 0.74          & 0.72          & 0.76          \\
%                                                                                     & Tweet-NLP               &                                                        & 0.79          & 0.5           & 0.15       &                                                        & 0.87          & 0.79          & 0.72          &                                                        & 0.86          & 0.74          & 0.83       &                                                        & 0.72          & 0.79          & 0.57          \\
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Asian\\ (2020)\end{tabular}}             & \ProjectNameTable{}                       & \multirow{3}{*}{179}                                   & \textbf{0.96} & \textbf{0.92} & \textbf{1} & \multirow{3}{*}{296}                                   & \textbf{0.96} & \textbf{0.93} & \textbf{0.99} & \multirow{3}{*}{331}                                   & \textbf{0.98} & \textbf{0.96} & \textbf{1} & \multirow{3}{*}{262}                                   & \textbf{0.98} & \textbf{0.97} & \textbf{1}    \\
%                                                                                     & BERT-base               &                                                        & 0.68          & 0.91          & 0.35       &                                                        & 0.84          & 0.79          & 0.8           &                                                        & 0.85          & 0.86          & 0.87       &                                                        & 0.87          & 0.88          & 0.92          \\
%                                                                                     & Tweet-NLP               &                                                        & 0.63          & 0.77          & 0.29       &                                                        & 0.84          & 0.84          & 0.72          &                                                        & 0.84          & 0.86          & 0.84       &                                                        & 0.85          & 0.91          & 0.86          \\
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Mask\\ (2020)\end{tabular}}              & \ProjectNameTable{}                       & \multirow{3}{*}{16}                                    & \textbf{1}    & \textbf{1}    & \textbf{1} & \multirow{3}{*}{64}                                    & \textbf{1}    & \textbf{1}    & \textbf{1}    & \multirow{3}{*}{249}                                   & \textbf{0.99} & \textbf{0.96} & \textbf{1} & \multirow{3}{*}{199}                                   & \textbf{0.99} & \textbf{0.98} & \textbf{1}    \\
%                                                                                     & BERT-base               &                                                        & 0.75          & 0             & 0          &                                                        & 0.79          & 0.78          & 0.39          &                                                        & 0.85          & 0.75          & 0.66       &                                                        & 0.8           & 0.75          & 0.86          \\
%                                                                                     & Tweet-NLP               &                                                        & 0.94          & 0.67          & \textbf{1} &                                                        & 0.86          & 0.85          & 0.61          &                                                        & 0.87          & 0.75          & 0.78       &                                                        & 0.84          & 0.8           & 0.88          \\
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Vaccine\\ (2020)\end{tabular}}           & \ProjectNameTable{}                       & \multirow{3}{*}{78}                                    & \textbf{0.97} & \textbf{0.93} & \textbf{1} & \multirow{3}{*}{114}                                   & \textbf{0.96} & \textbf{0.89} & \textbf{1}    & \multirow{3}{*}{104}                                   & \textbf{0.98} & \textbf{0.95} & \textbf{1} & \multirow{3}{*}{226}                                   & \textbf{0.99} & \textbf{0.97} & \textbf{1}    \\
%                                                                                     & BERT-base               &                                                        & 0.76          & 0.92          & 0.38       &                                                        & 0.78          & 0.68          & 0.7           &                                                        & 0.85          & 0.79          & 0.83       &                                                        & 0.84          & 0.75          & 0.79          \\
%                                                                                     & Tweet-NLP               &                                                        & 0.72          & 0.77          & 0.35       &                                                        & 0.75          & 0.6           & 0.83          &                                                        & 0.8           & 0.75          & 0.73       &                                                        & 0.88          & 0.83          & 0.82          \\
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}US Capitol\\ (2021)\end{tabular}}        & \ProjectNameTable{}                       & \multirow{3}{*}{311}                                   & \textbf{0.99} & \textbf{0.98} & \textbf{1} & \multirow{3}{*}{112}                                   & \textbf{1}    & \textbf{1}    & \textbf{1}    & \multirow{3}{*}{158}                                   & \textbf{1}    & \textbf{1}    & \textbf{1} & \multirow{3}{*}{123}                                    & \textbf{0.99} & \textbf{1}    & \textbf{0.98} \\
%                                                                                     & BERT-base               &                                                        & 0.68          & 0.79          & 0.31       &                                                        & 0.85          & 0.85          & 0.83          &                                                        & 0.82          & 0.85          & 0.76       &                                                        & 0.84          & 0.78          & 0.89          \\
%                                                                                     & Tweet-NLP               &                                                        & 0.63          & 0.7           & 0.16       &                                                        & 0.83          & 0.79          & 0.87          &                                                        & 0.82          & 0.87          & 0.72       &                                                        & 0.78          & 0.75          & 0.79          \\
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Russia\\ -Ukraine\\ (2022)\end{tabular}} & \ProjectNameTable{}                       & \multirow{3}{*}{158}                                   & \textbf{1}    & \textbf{1}    & \textbf{1} & \multirow{3}{*}{190}                                   & \textbf{0.99} & \textbf{0.98} & \textbf{1}    & \multirow{3}{*}{192}                                   & \textbf{0.99} & \textbf{0.99} & \textbf{1} & \multirow{3}{*}{60}                                   & \textbf{1}    & \textbf{1}    & \textbf{1}    \\
%                                                                                     & BERT-base               &                                                        & 0.8           & 0.85          & 0.37       &                                                        & 0.8           & 0.72          & 0.62          &                                                        & 0.82          & 0.82          & 0.81       &                                                        & 0.83          & 0.82          & 0.87          \\
%                                                                                     & Tweet-NLP               &                                                        & 0.77          & 0.92          & 0.24       &                                                        & 0.84          & 0.82          & 0.65          &                                                        & 0.86          & 0.88          & 0.84       &                                                        & 0.85          & 0.89          & 0.81         
% \\

% \bottomrule
% \end{tabular}%
\begin{tabular}{cccccccccccccccccc}
\toprule
\multirow{3}{*}{\textbf{Wave Type}}                                                           & \multirow{3}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Quarter 1 (Jan-Mar)}}                                                                    & \multicolumn{4}{c}{\textbf{Quarter 2 (Apr-Jun)}}                                                                       & \multicolumn{4}{c}{\textbf{Quarter 3 (Jul-Sep})}                                                                    & \multicolumn{4}{c}{\textbf{Quarter 4 (Oct-Dec)}}                                                                       \\
\cmidrule(r){3-6} \cmidrule(r){7-10} \cmidrule(r){11-14} \cmidrule(r){15-18}     
                                                                                    &                         & \textbf{\begin{tabular}[c]{@{}c@{}}\# of\\ Tweets\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Acc-\\ uracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Prec-\\ ision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rec-\\ all\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# of\\ Tweets\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Acc-\\ uracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Prec-\\ ision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rec-\\ all\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# of\\ Tweets\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Acc-\\ uracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Prec-\\ ision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rec-\\ all\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\# of\\ Tweets\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Acc-\\ uracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Prec-\\ ision\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Rec-\\ all\end{tabular}} \\
\midrule
\multicolumn{18}{c}{\textbf{- Overall Results -}}\\
\midrule
\multirow{3}{*}{
\begin{tabular}[c]{@{}c@{}}Total\\ (2020-2022)\end{tabular}
} 
& \ProjectNameTable{} & \multirow{3}{*}{928} & \textbf{0.99} & \textbf{0.96}    & \textbf{0.99} & 
\multirow{3}{*}{893} & \textbf{0.98} & \textbf{0.96} & \textbf{0.99}    
& \multirow{3}{*}{1148} & \textbf{0.99} & \textbf{0.97} & \textbf{0.99} & 
\multirow{3}{*}{1031} & \textbf{0.99}    & \textbf{0.98}    & \textbf{0.99}    \\
& BERT-base & & 0.74 & 0.81& 0.34& & 0.82& 0.76& 0.71& &0.84 & 0.82& 0.79& & 0.83& 0.86&0.8 \\
& Tweet-NLP & &0.7 &0.73 &0.23 & & 0.83&0.79 &0.77 & &0.84 & 0.83& 0.8& &0.83 &0.84 &0.8 \\
\midrule
\multicolumn{18}{c}{\textbf{- Category-wise Results -}}\\
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Ageism\\ (2020)\end{tabular}}            & \ProjectNameTable{}                       & \multirow{3}{*}{186}                                   & \textbf{0.99} & \textbf{0.97} & \textbf{0.99} & \multirow{3}{*}{117}                                   & \textbf{0.99}    & \textbf{0.99}    & \textbf{0.99}    & \multirow{3}{*}{114}                                   & \textbf{0.99}    & \textbf{0.99}    & \textbf{0.99} & \multirow{3}{*}{161}                                   & \textbf{0.99}    & \textbf{0.99}    & \textbf{0.99}    \\
                                                                                    & BERT-base               &                                                        & 0.82          & 0.6           & 0.44       &                                                        & 0.8           & 0.68          & 0.53          &                                                        & 0.79          & 0.68          & 0.6        &                                                        & 0.74          & 0.72          & 0.76          \\
                                                                                    & Tweet-NLP               &                                                        & 0.79          & 0.5           & 0.15       &                                                        & 0.87          & 0.79          & 0.72          &                                                        & 0.86          & 0.74          & 0.83       &                                                        & 0.72          & 0.79          & 0.57          \\
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Asian\\ (2020)\end{tabular}}             & \ProjectNameTable{}                       & \multirow{3}{*}{179}                                   & \textbf{0.96} & \textbf{0.92} & \textbf{0.99} & \multirow{3}{*}{296}                                   & \textbf{0.96} & \textbf{0.93} & \textbf{0.99} & \multirow{3}{*}{331}                                   & \textbf{0.98} & \textbf{0.96} & \textbf{0.99} & \multirow{3}{*}{262}                                   & \textbf{0.98} & \textbf{0.97} & \textbf{0.99}    \\
                                                                                    & BERT-base               &                                                        & 0.68          & 0.91          & 0.35       &                                                        & 0.84          & 0.79          & 0.8           &                                                        & 0.85          & 0.86          & 0.87       &                                                        & 0.87          & 0.88          & 0.92          \\
                                                                                    & Tweet-NLP               &                                                        & 0.63          & 0.77          & 0.29       &                                                        & 0.84          & 0.84          & 0.72          &                                                        & 0.84          & 0.86          & 0.84       &                                                        & 0.85          & 0.91          & 0.86          \\
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Mask\\ (2020)\end{tabular}}              & \ProjectNameTable{}                       & \multirow{3}{*}{16}                                    & \textbf{0.99}    & \textbf{0.99}    & \textbf{0.99} & \multirow{3}{*}{64}                                    & \textbf{0.99}    & \textbf{0.99}    & \textbf{0.99}    & \multirow{3}{*}{249}                                   & \textbf{0.99} & \textbf{0.96} & \textbf{0.99} & \multirow{3}{*}{199}                                   & \textbf{0.99} & \textbf{0.98} & \textbf{0.99}    \\
                                                                                    & BERT-base               &                                                        & 0.75          & 0             & 0          &                                                        & 0.79          & 0.78          & 0.39          &                                                        & 0.85          & 0.75          & 0.66       &                                                        & 0.8           & 0.75          & 0.86          \\
                                                                                    & Tweet-NLP               &                                                        & 0.94          & 0.67          & \textbf{0.99} &                                                        & 0.86          & 0.85          & 0.61          &                                                        & 0.87          & 0.75          & 0.78       &                                                        & 0.84          & 0.8           & 0.88          \\
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Vaccine\\ (2020)\end{tabular}}           & \ProjectNameTable{}                       & \multirow{3}{*}{78}                                    & \textbf{0.97} & \textbf{0.93} & \textbf{0.99} & \multirow{3}{*}{114}                                   & \textbf{0.96} & \textbf{0.89} & \textbf{0.99}    & \multirow{3}{*}{104}                                   & \textbf{0.98} & \textbf{0.95} & \textbf{0.99} & \multirow{3}{*}{226}                                   & \textbf{0.99} & \textbf{0.97} & \textbf{0.99}    \\
                                                                                    & BERT-base               &                                                        & 0.76          & 0.92          & 0.38       &                                                        & 0.78          & 0.68          & 0.7           &                                                        & 0.85          & 0.79          & 0.83       &                                                        & 0.84          & 0.75          & 0.79          \\
                                                                                    & Tweet-NLP               &                                                        & 0.72          & 0.77          & 0.35       &                                                        & 0.75          & 0.6           & 0.83          &                                                        & 0.8           & 0.75          & 0.73       &                                                        & 0.88          & 0.83          & 0.82          \\
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}US Capitol\\ (2021)\end{tabular}}        & \ProjectNameTable{}                       & \multirow{3}{*}{311}                                   & \textbf{0.99} & \textbf{0.98} & \textbf{0.99} & \multirow{3}{*}{112}                                   & \textbf{0.99}    & \textbf{0.99}    & \textbf{0.99}    & \multirow{3}{*}{158}                                   & \textbf{0.99}    & \textbf{0.99}    & \textbf{0.99} & \multirow{3}{*}{123}                                    & \textbf{0.99} & \textbf{0.99}    & \textbf{0.98} \\
                                                                                    & BERT-base               &                                                        & 0.68          & 0.79          & 0.31       &                                                        & 0.85          & 0.85          & 0.83          &                                                        & 0.82          & 0.85          & 0.76       &                                                        & 0.84          & 0.78          & 0.89          \\
                                                                                    & Tweet-NLP               &                                                        & 0.63          & 0.7           & 0.16       &                                                        & 0.83          & 0.79          & 0.87          &                                                        & 0.82          & 0.87          & 0.72       &                                                        & 0.78          & 0.75          & 0.79          \\
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Russia\\ -Ukraine\\ (2022)\end{tabular}} & \ProjectNameTable{}                       & \multirow{3}{*}{158}                                   & \textbf{0.99}    & \textbf{0.99}    & \textbf{0.99} & \multirow{3}{*}{190}                                   & \textbf{0.99} & \textbf{0.98} & \textbf{0.99}    & \multirow{3}{*}{192}                                   & \textbf{0.99} & \textbf{0.99} & \textbf{0.99} & \multirow{3}{*}{60}                                   & \textbf{0.99}    & \textbf{0.99}    & \textbf{0.99}    \\
                                                                                    & BERT-base               &                                                        & 0.8           & 0.85          & 0.37       &                                                        & 0.8           & 0.72          & 0.62          &                                                        & 0.82          & 0.82          & 0.81       &                                                        & 0.83          & 0.82          & 0.87          \\
                                                                                    & Tweet-NLP               &                                                        & 0.77          & 0.92          & 0.24       &                                                        & 0.84          & 0.82          & 0.65          &                                                        & 0.86          & 0.88          & 0.84       &                                                        & 0.85          & 0.89          & 0.81         
\\

\bottomrule
\end{tabular}%
}
\caption{Comparing \ProjectNameTable{}  against the existing  benchmarks.}
\vspace{-5mm}
\label{tab:violations_compare_baseline}
\end{table*}
